Improved Evolutionary Algorithms for Submodular Maximization with Cost Constraints

We present an evolutionary algorithm evo-SMC for the problem of Submodular Maximization under Cost constraints (SMC). Our algorithm achieves $1/2$-approximation with a high probability $1-1/n$ within $\mathcal{O}(n^2K_{\beta})$ iterations, where $K_{\beta}$ denotes the maximum size of a feasible solution set with cost constraint $\beta$. To the best of our knowledge, this is the best approximation guarantee offered by evolutionary algorithms for this problem. We further refine evo-SMC, and develop st-evo-SMC. This stochastic version yields a significantly faster algorithm while maintaining the approximation ratio of $1/2$, with probability $1-\epsilon$. The required number of iterations reduces to $\mathcal{O}(nK_{\beta}\log{(1/\epsilon)}/p)$, where the user defined parameters $p \in (0,1]$ represents the stochasticity probability, and $\epsilon \in (0,1]$ denotes the error threshold. Finally, the empirical evaluations carried out through extensive experimentation substantiate the efficiency and effectiveness of our proposed algorithms. Our algorithms consistently outperform existing methods, producing higher-quality solutions.

==> 7.1-PO.tex <==
\section{Constrained Pareto Optimization}
\label{sec:app-PO}

% Algorithm \ref{alg:po} solves the submodualr maximization problem with a budget $\beta$. Instead of solely optimizing submodular function $f$, it optimize a surrogate function $g$, define in Definition \ref{def:g}. It first initializes a $2 \times P$ matrix $S$ with empty sets, where the first column of $S$ is $S[0,]$ serves to store the temporary best solution at an iteration with respect to $f$ and similarly the second column is for $g$. For example, $S[1,i]$ is the best set achieving best $g$ value with cardinality no greater than $i$ at the end of iteration $t-1$. For each iteration, the algorithm randomly select a set from the best of $g$ value, then mutate it. The \Mutate procedure (Algorithm \ref{alg:mutate}) removes or adds an element with probability $1/n$. If the returned set from \Mutate satisfies the constraints and has a higher $f$ value or $g$ value and a smaller size, the algorithm will update the $S$ matrix accordingly (line 9-13). At the end, the algorithm outputs the best of $y^*$ and sets in $S$. 


\begin{algorithm}
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \Input{$f:2^V \rightarrow \mathbb{R}_{\geq 0}, c: 2^V \rightarrow \mathbb{R}_{\geq 0}$\\ total number of iterations $T\in \mathbb{Z}_{> 0}, $ cost constraint $\beta \in \mathbb{R}_{> 0}$}
    \Output{\\ $\argmax_{X \in \{F_0,\cdots,F_{n-1},G_0, \cdots, G_{n-1},G_0', \cdots, G_{n-1}'\}}f(X)$}
    $F_j \gets \emptyset, G_j \gets \emptyset, G_j' \gets \emptyset$ for all $j \in [0, n-1]$\\
    \For{$t \gets 1$ \textbf{to} $T$} {
        $S \gets \text{Random}(\{F_0,\cdots,F_{n-1},G_0, \cdots, G_{n-1}\})$\\
        $S' \gets$ \Call{\Mutate}{$S$}\\
        $i \gets |S'|$\\
        \If{$c(S') \leq \beta$}{
            \If{$f(F_i) < f(S')$}{
                $F_i \gets S'$
            }
            \If{$g(G_i) < g(S')$}{
                $G_i \gets S'$\\
                $G_i' \gets G_i \cup \{v\}$, $v=\argmax_{e \in V\setminus G_i}f(v \mid G_i)$
            }
        }
        
    }
    \caption{\textsc{c-PO}}
    % \label{alg:po}
\end{algorithm}

\begin{algorithm}
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \Input{$S$}
    \Output{$S'$}
    
    \For{$x \in V$} {
        
        \eIf{$x \in S$} {
            $S'=S \setminus\{x\}$ with probability $1/n$
        }
        {
            $S'=S\cup \{x\}$ with probability $1/n$
        }
    }
    \caption{\Mutate}
    % \label{alg:mutate}
\end{algorithm}



\begin{theorem}
    With a submodular function $f$, a cost function $c$, a cost constraint $\beta$, let $\OPT_{\beta}=\argmax\{f(X) \mid X\subseteq V, c(X)\leq \beta\}$. If $K_{\beta}=\max\{ |X| \mid X \subseteq V \wedge c(X) \leq \beta \}$, then after $T\geq \max\{4en^2K_{\beta}, 16enK_{\beta}\log n\}$ iterations,  Algorithm \ref{alg:po} outputs $X$ and admits $\frac{1}{2}$-approximation with high probability.
    \[f(X) \geq \frac{1}{2}f(\OPT_{\beta})\] 
% \label{th:po}
\end{theorem}



\begin{proof}

Our theoretical analysis of this theorem is based on function $g$. The definition is:

\begin{definition}[$g(X)$] For a set $X \subseteq U$
\[ g(X) =
  \begin{cases}
    f(X)/c(X)       & \quad \text{if } |X|\geq 1\\
    f(X)  & \quad \text{else }
  \end{cases}
\]
    % \label{def:g}

\end{definition}

% \begin{definition}[$Domination~Relations$] For sets $X, Y \subseteq V$, define
% \[ X \stackrel{f}{\preceq} Y \quad \text{if~} f(Y) \geq f(X) \wedge c(Y) \leq c(X) \] 
% \[ X \stackrel{g}{\preceq} Y \quad \text{if~} g(Y) \geq g(X) \wedge c(Y) \leq c(X) \] 
% \label{def:dom}

% \end{definition}




We define $\omega$ to keep track of the size of a candidate set that we want the algorithm to select.

\begin{definition}[$\omega$] 
$\omega=0$ at the beginning of the algorithm, $\omega(0)=0$. $\omega$ is incremented if the following three conditions are met at an iteration $t$. Then $\omega(t)=\omega(t-1)+1$.
\begin{enumerate}
    \item A specific set $S=G_{\omega(t-1)}$ is selected for mutation at line 3 of Algorithm \ref{alg:po}.
    \item There is exactly one element added to $S$ during \Mutate procedure, say $S'=S \cup \{a\}$, where $a = \argmax_{e\in \OPT_{\beta} \setminus (S \cup \{o^*\})} \frac{f(e|S)}{c(e)}$, where $o^* = \argmax_{e \in \OPT_{\beta}} c(e)$.
\end{enumerate}
% \label{def:w}

\end{definition}

\begin{observation}
$\omega$ is incremented with a probability at least $\frac{1}{2en^2}$ and it is independent of the iteration $t$.
% \label{obs:probability}
\end{observation}
\begin{proof}
Define event $R$: at iteration $t$, $\omega$ increments. Event $R$ happens when the above three conditions are met. A set $S$ is selected and considered to mutate with a probability $\frac{1}{2n}$ (line 3 of Algorithm \ref{alg:po}). Since every element of $S$ is flipped with probability $\frac{1}{n}$, the probability that element $a = \argmax_{e\in \OPT_{\beta} \setminus (S \cup \{o^*\})} \frac{f(e|S)}{c(e)}$ was flipped is $\frac{1}{n}\cdot (1-\frac{1}{n})^{n-1}$. The mutation process is independent of $t$.

Therefore, 
\begin{align*}
    \Pr[R] &= \frac{1}{2n} \cdot \frac{1}{n}\cdot (1-\frac{1}{n})^{n-1}\\
    &\geq \frac{1}{2en^2}
\end{align*}
    
\end{proof}

\begin{remark}
    $\omega$ is used to control the size of a candidate set.\\
    $\omega(t-1)$ is the size of a candidate set at iteration $t$.
\end{remark}

\begin{definition}[$X_{t}$] At the beginning of iteration $t$, $X_{t-1}$ is the solution set where $X_{t-1} = G_{\omega(t-1)}$. At the end of iteration $t$, $X_{t}$ is the the set where $X_{t} = G_{\omega(t)}$.


    
% \label{def:Xt}
\end{definition}


\begin{lemma}
    In Algorithm \ref{alg:po}, at the beginning of iteration $t$, assume set $S=X_{t-1}$ is the candidate set selected for mutation, which satisfies $c(S) \leq c(\OPT_{\beta})-c(o^*)$ where  $o^* = \argmax_{e \in \OPT_{\beta}} c(e)$. If a good mutation happened, i.e., the algorithm added the element $v = \argmax_{e \in \OPT_{\beta} \setminus (S \cup \{o^*\})} \{ \frac{f(e|S)}{c(e)}\} $ to $S$, we have: 

    \[ f(S \cup \{v\})-f(S) \geq \frac{c(v)}{c(\OPT_{\beta})-c(o^*)}(f(\OPT_{\beta})-f(S\cup \{o^*\})) \]
% \label{lem:greedy}
\end{lemma}

\begin{proof}

Since $v = \argmax_{e \in \OPT_{\beta} \setminus (S \cup \{o^*\})} \{ \frac{f(e|S)}{c(e)} \} $, for every $u\in \OPT_{\beta}\setminus(S\cup \{o^*\})$,
\begin{equation}
    % \label{eq:greedy-marginal}
    \frac{f(v|S)}{c(e)} \geq \frac{f(u|S)}{c(u)}
\end{equation}

    \begin{align*}
        f(\OPT_{\beta})-f(S \cup \{o^*\})  & \leq f((\OPT_{\beta} \cup S \cup \{o^*\}) \cup S ) - f(S) \quad\quad \mbox{monotonicity}\\
        & \leq \sum_{u \in \OPT_{\beta}\setminus(S \cup \{o^*\})} f(u | S \cup \{o^*\} )\\
        & \leq \sum_{u \in \OPT_{\beta}\setminus(S \cup \{o^*\})} f(u | S ) \quad\quad\quad \mbox{submodularity}\\
        & \leq \sum_{u \in \OPT_{\beta}\setminus(S \cup \{o^*\})} \frac{f(v|S)}{c(v)} \cdot c(u) \quad\quad \mbox{from Eq. (\ref{eq:greedy-marginal})}\\
        & = \frac{f(v|S)}{c(v)} \sum_{u \in \OPT_{\beta}\setminus(S \cup \{o^*\})} c(u)\\
        &\leq \frac{f(v|S)}{c(v)} \left(c(\OPT_{\beta})-c(o^*)\right)
    \end{align*}
We finish the proof by rearranging the above equation.
\end{proof}




To finish the proof of Theorem \ref{th:po}, we need to prove the following lemma.

\begin{lemma}
    For any iteration $1 \leq t \leq T$, let $X_t$ be the set with size $\omega(t)$ at the end of iteration $t$, then we have:
    \[ f(X_t) \geq \frac{c(X_t)}{2(c(\OPT_{\beta})-c(o^*))}f(\OPT_{\beta}) \]
% \label{lem:Xt}
\end{lemma}

\begin{proof}
    We prove this lemma by induction.

    \medskip
    \noindent
    \textbf{Basis Steps: } For the first iteration $t=1$ of algorithm \ref{alg:po}, we have two cases.

    \begin{itemize}
        \item \textbf{Case B-1}: $\omega$ is not incremented, then we have $\omega(1)=\omega(0)=0$, $|X_0|=|X_1|=\omega(1)=0$ and $X_1=\emptyset$. So we have
        \[f(X_1)=0 \geq \frac{c(X_1)}{2(c(\OPT_{\beta})-c(o^*))}f(\OPT_{\beta})=0\]
        
        \item \textbf{Case B-2}: $\omega$ is incremented, then we have $\omega(1)=\omega(0)+1=1$. \\
        Since this is the first iteration, $X_0=\emptyset$. By Definition \ref{def:w}, $|X_1|=1$ and the two conditions are satisfied. Assume that the element in condition 3 of Definition \ref{def:w} is $v$. Then, $X_1=\{v\}$, apply Lemma \ref{lem:greedy}, we have
        % \[ f(X_1) -f(X_0) \geq  \frac{c(X_1)}{2(c(\OPT_{\beta})-c(o^*))}f(\OPT_{\beta})\]
        \begin{align*}
            f(X_1) &= f(X_1) - f(X_0) \\
            &= f(\{v\}) - f(\emptyset) \\
            &\geq \frac{c(v)}{c(\OPT_{\beta})-c(o^*)}(f(\OPT_{\beta})-f(\{o^*\})) \quad\quad \mbox{due to Lem. \ref{lem:greedy} with $S=X_0=\emptyset$}\\
            & \geq \frac{c(v)}{2(c(\OPT_{\beta})-c(o^*))}f(\OPT_{\beta}) \quad\quad \mbox{assume $f(\{o^*\}) < \frac{1}{2}f(\OPT_{\beta})$ }\\
            &= \frac{c(X_1)}{2(c(\OPT_{\beta})-c(o^*))}f(\OPT_{\beta}) \quad\quad \mbox{due to $X_1=\{v\}$}
        \end{align*}

    \end{itemize}
    Thus, Lemma \ref{lem:Xt} holds for $t=1$. 
    Next suppose at iteration $t-1$ Lemma \ref{lem:Xt} is true, we prove for iteration $t$ it still holds. 
    % Before that, we give a useful observation.
    % \begin{observation} For any iteration $t>1$,
    % \[g(X_t) \geq g(X_{t-1}) ~~ and ~~ f(F_{\omega(t)}) \geq f(F_{\omega(t-1)})\]
    %        \label{obs:g1}
    % \end{observation}
    % \begin{proof}
    %     By line 10-11 of the algorithm \ref{alg:po}, $X_i$ is always no worse than $X_j$ for all $1\leq j<i\leq T$.
    % \end{proof}
    
\noindent        
\textbf{Induction Steps: } For iteration $t>1$. We assume Lemma \ref{lem:Xt} holds for iteration $t-1$.
\begin{equation}
    % \label{eq:IH-cpo}
    f(X_{t-1}) \geq \frac{c(X_{t-1})}{2(c(\OPT_{\beta})-c(o^*))}f(\OPT_{\beta})
\end{equation}

We also have two case. 
\begin{itemize}
    \item \textbf{Case I-1:} $\omega$ is not incremented, then we have $\omega(t)=\omega(t-1)$. \\
    By Definition \ref{def:g}, we have $|X_t|=|X_{t-1}|=\omega({t-1})$ and
    \[g(X_t) \geq g(X_{t-1}) \Rightarrow \frac{f(X_t)}{c(X_t)} \geq \frac{f(X_{t-1})}{c(X_{t-1})}\]
    Thus,
    \begin{align*}
        f(X_t) &\geq \frac{c(X_t)}{c(X_{t-1})}f(X_{t-1})\\
        &\geq \frac{c(X_t)}{c(X_{t-1})}\cdot \frac{c(X_{t-1})}{2(c(\OPT_{\beta})-c(o^*))}f(\OPT_{\beta}) \quad\quad\mbox{due to I.H.}\\
        &=\frac{c(X_t)}{2(c(\OPT_{\beta})-c(o^*))}f(\OPT_{\beta})
    \end{align*}
    The last inequality is due to the induction hypothesis. This concludes the proof of Lemma \ref{lem:Xt} for this case.  
    
    \item \textbf{Case I-2:} $\omega$ is incremented, then we have $\omega(t)=\omega(t-1)+1$. In this case, $X_{t-1}$ is selected for mutation and the mutation gives $|X_t|=|X_{t-1} \cup \{v\}|$ where $v = \argmax_{u\in \OPT_{\beta} \setminus (X_{t-1} \cup  \{o^*\})}\{ \frac{f(u|X_{t-1})}{c(u)} \}$.

    \begin{itemize}
        \item \textit{Case I-2.1:} $c(X_{t-1}) \geq c(\OPT_{\beta}) - c(o^*)$\\
        We prove in this case the algorithm admits a $1/2$-approximation at the end of iteration $t-1$.
        \begin{align*}
            f(F_{\omega(t)}) &\geq f(X_{t-1} \cup \{v\}) \geq f(X_{t-1})\\ &\geq \frac{c(X_{t-1})}{2(c(\OPT_{\beta})-c(o^*))}f(\OPT_{\beta}) \quad\quad\mbox{due to I.H.}\\
            &\geq \frac{1}{2} f(\OPT_{\beta})
        \end{align*}
        
        \item \textit{Case I-2.2:} $c(X_{t-1}) < c(\OPT_{\beta}) - c(o^*)$
        
        \begin{claim}
        W.l.o.g., for any iteration $t<T$, we can safely assume: 
        \begin{equation}
        % \label{eq:lem-assumption}
            f(X_{t-1} \cup \{o^*\}) < \frac{1}{2} f(\OPT_{\beta})
        \end{equation}
        Otherwise, at the end of iteration $t-1$, the algorithm already admits a $1/2$-approximation.
    \end{claim}
    \begin{proof}
        Suppose $f(X_{t-1} \cup \{o^*\}) \geq \frac{1}{2} f(\OPT_{\beta})$, 
        We argue this claim in two cases: 
        
        (1) If $o^* \in X_{t-1}$, then $X_{t-1} \cup \{o^*\} = X_{t-1}$. In this case, $f(X_{t-1}) \geq \frac{1}{2} f(\OPT_{\beta})$, which is guaranteed $1/2$-approximation. 
        
        (2) If $o^* \notin X_{t-1}$, then due to line 12 of the algorithm, there exists $|G'_{w(t-1)}| = |X_{t-1} \cup \{o^*\}|$ and $f(G'_{w(t-1)}) \geq f(X_{t-1} \cup \{o^*\}) \geq \frac{1}{2} f(\OPT_{\beta})$. If $c(o^*) > \beta - c(X_{t-1})$, then $c(X_{t-1}) > \beta - c(o^*) \geq c(\OPT_{\beta}) - c(o^*)$, which is a contradiction with the Case 2.2 condition.
    \end{proof}
        
    Since $g(\cdot)$ is non-decreasing on the same cardinality set, we have
    \[g(X_t) \geq g(X_{t-1} \cup \{v\}) \Rightarrow \frac{f(X_t)}{c(X_t)} \geq \frac{f(X_{t-1}\cup \{v\})}{c(X_{t-1}\cup \{v\})}\]
    
    Then by rearranging Lemma \ref{lem:greedy} where $S=X_{t-1}$, we have
    \begin{align*}
    &f(X_{t-1} \cup \{v\})\\
    &\geq \frac{c(v)}{c(\OPT_{\beta})-c(o^*)} \left(f(\OPT_{\beta})-f(X_{t-1} \cup \{o^*\}) \right)+f(X_{t-1})\\
        &= \frac{c(v)}{c(\OPT_{\beta})-c(o^*)} f(\OPT_{\beta}) + f(X_{t-1}) - \frac{c(v)}{c(\OPT_{\beta})-c(o^*)}f(X_{t-1} \cup \{o^*\})\\
        &\geq \frac{c(v)}{c(\OPT_{\beta})-c(o^*)} f(\OPT_{\beta}) + f(X_{t-1}) - \frac{c(v)}{2(c(\OPT_{\beta})-c(o^*))}f(\OPT_{\beta}) \quad\quad \mbox{from Eq. (\ref{eq:lem-assumption})}\\
        &=\frac{c(v)}{2(c(\OPT_{\beta})-c(o^*))}f(\OPT_{\beta}) + f(X_{t-1})\\
        &\geq \frac{c(v)}{2(c(\OPT_{\beta})-c(o^*))}f(\OPT_{\beta}) + \frac{c(X_{t-1})}{2(c(\OPT_{\beta})-c(o^*))}f(\OPT_{\beta}) \quad\quad \mbox{due to Induction Hypothesis}\\
        &=\frac{c(X_{t-1} \cup \{v\})}{2(c(\OPT_{\beta})-c(o^*))}f(\OPT_{\beta})\\
    \end{align*}

    Therefore, 
    \[ f(X_t) \geq \frac{c(X_t)}{c(X_{t-1}\cup \{v\})} f(X_{t-1}\cup \{v\}) \geq \frac{c(X_{t})}{2(c(\OPT_{\beta})-c(o^*))}f(\OPT_{\beta}) \]
    \end{itemize}
\end{itemize}
We conclude the proof of Lemma \ref{lem:Xt}.
\end{proof}

At iteration $t$, the algorithm selected $X_{t-1}$ for mutation. If at the end of iteration $t$, $\omega$ is incremented, we analyze the cost of $c(X_{t-1} \cup \{v\})$. 

% We have the following claim.

% \begin{claim}
%     \label{claim:feasibility}
%     At any iteration $t$, the algorithm selected $X_{t-1}$ for mutation resulting in increment of $\omega$, if $c(X_{t-1} \cup \{v\}) > \beta$ where $v = \argmax_{e \in \OPT_{\beta} \setminus (X_{t-1} \cup \{o^*\})} \{ \frac{f(e|X_{t-1})}{c(e)}\}$, then $f(X_{t-1}) \geq \frac{1}{2} f(\OPT_{\beta})$
% \end{claim}
% \begin{proof}
%     Function $c$ is modular, so $c(X_{t-1} \cup \{v\}) = c(X_{t-1}) + c(v) > \beta$. Then 
%     \[c(X_{t-1}) > \beta - c(v) \geq c(\OPT_{\beta}) - c(o^*)\]
%     This inequality holds from $\beta \geq c(\OPT_{\beta})$ and $c(v) \leq c(o^*)$. By Lemma~\ref{lem:Xt}, if $c(X_{t-1}) > c(\OPT_{\beta}) - c(o^*)$, the algorithm already admits $1/2$-approximation for $f(X_{t-1})$.
% \end{proof}

Therefore, due to the Case 2.1 analysis of Lemma \ref{lem:Xt}, we next assume that $c(X_{t-1} \cup \{v\}) \leq \beta$ for $v = \argmax_{e \in \OPT_{\beta} \setminus (X_{t-1} \cup \{o^*\})} \{ \frac{f(e|X_{t-1})}{c(e)}\}$. 


\begin{figure*}[htbp]
\centering
\includegraphics[width=0.8\textwidth]{illustration.pdf}
  \caption{An Illustration to the costs}
  % \label{flowchart}
\end{figure*}

\begin{enumerate}
    \item \textcolor{blue}{$c(X_{t-1}) < c(X_{t-1} \cup \{v\}) < c(\OPT_{\beta})-c(o^*)$.}\\
    $\bullet$ If there does not exist $X_{t-1} \cup \{v\}$ such that $c(X_{t-1} \cup \{v\}) \geq c(\OPT_{\beta})-c(o^*)$, then the algorithm will output the optimal solution. The reason is that $\omega(t)$ can be up to $n$, i.e., $|X_t|=|X_{t-1} \cup \{v\}|$ can be as large as $n$. \\
    Otherwise, the algorithm can keep running until $c(X_{t-1} \cup \{v\}) \geq c(\OPT_{\beta})-c(o^*)$.
    
    $\bullet$ Also, the cost of a new candidate element $e \in \OPT_{\beta} \setminus (X_{t-1} \cup \{o^*\})$ can be up to $\beta - c(X_{t-1}) > c(\OPT_{\beta}) - [c(\OPT_{\beta})-c(o^*)] = c(o^*)$. Therefore, every element $e \in \OPT_{\beta} \setminus X_{t-1}$ is feasible to $X_{t-1}$. 
    \begin{itemize}
        \item[$\circ$] If $o^* \notin X_{t-1}$, then every $e \in \OPT_{\beta} \setminus (X_{t-1} \cup \{o^*\})$ is feasible for $X_{t-1}$. The algorithm can keep adding them until $c(X_{t-1} \cup \{v\}) \geq c(\OPT_{\beta})-c(o^*)$. If the condition $c(X_{t-1} \cup \{v\}) \geq c(\OPT_{\beta})-c(o^*)$ cannot be satisfied after adding every $e \in \OPT_{\beta} \setminus (X_{t-1} \cup \{o^*\})$, which implies that $\OPT_{\beta} \setminus \{o^*\} \subseteq X_{t-1} \cup \{v\}$. We assumed that $f(\{o^*\}) < 1/2 f(\OPT_{\beta})$, therefore, by monotonicity and submodularity, we have
        \[f(X_t) \geq f(X_{t-1} \cup \{v\}) \geq f(\OPT_{\beta} \setminus \{o^*\}) \geq f(\OPT_{\beta}) - f(\{o^*\}) \geq 1/2 f(\OPT_{\beta})\]
        
        \item[$\circ$] If $o^* \in X_{t-1}$, similar analysis is applicable as above. Every $e \in \OPT_{\beta} \setminus (X_{t-1} \cup \{o^*\})$, i.e., $e \in \OPT_{\beta} \setminus X_{t-1}$  is feasible for $X_{t-1}$. The algorithm can keep adding them until $c(X_t) \geq c(\OPT_{\beta})-c(o^*)$. If the condition $c(X_{t-1} \cup \{v\}) \geq c(\OPT_{\beta})-c(o^*)$ cannot be satisfied when $\omega(t)=n$, the algorithm outputs the optimal solution (the universal set $V$).
    \end{itemize}
    
    \item \textcolor{teal}{$c(X_{t-1}) < c(\OPT_{\beta})-c(o^*) \leq c(X_{t-1} \cup \{v\}) \leq \beta $}\\
    In this case, Lemma \ref{lem:Xt} indicates $f(X_t) \geq 1/2 f(\OPT_{\beta})$.
    
    \item \textcolor{brown}{$c(X_{t-1}) < c(\OPT_{\beta})-c(o^*) < \beta < c(X_{t})$} does not exist.\\
    If this exists, $c(X_{t-1} \cup \{v\}) > \beta$ is an infeasible solution, which was discarded by the algorithm (line 6).
\end{enumerate}

We will wrap up the proof of this theorem by bounding the number of iterations $T$. 
\begin{lemma}[Chernoff Bound]
    For independent $0-1$ variables $Y_1, \cdots, Y_T$ with the same expectation (mean) and $Y=\sum_{i=1}^T Y_i$. If $\E[Y]=\mu$, for a real number $\eta \in (0,1)$, 
    \[\Pr[Y \leq (1-\eta)\mu] \leq e^{-\eta^2\mu/2}\]
\end{lemma}

\begin{lemma}
    In Algorithm \ref{alg:po}, define variable $Y_i$ for iteration $1\leq i \leq T$, where $T\geq \max\{2en^2K, 8enK\log n\}$
    \[ Y_i =
      \begin{cases}
        ~~ 1      & \quad \text{if } \omega(i)=\omega(i-1)+1\\
        ~~ 0  & \quad \text{if } \omega(i)=\omega(i-1)
      \end{cases}
    \]
    Suppose the maximum size of the solution set is $K$, then
    \[ \Pr[\sum_{i=1}^T Y_i < K_{\beta}] \leq \frac{1}{n} \]
\end{lemma}
\begin{proof}
    Observation \ref{obs:probability} gives the lower bound probability of $Y_i=1$ for an iteration $i$. Therefore, $\mu = \E[Y] = \E[\sum_{i=1}^T Y_i] = T \rho \geq T\cdot \frac{1}{2en^2}$. It is trivial that $Y_i's$ are independent and take binary values with identical expectations, so we can apply Chernoff bound.
    
    \begin{align*}
        \Pr[\sum_{i=1}^T Y_i < K_{\beta}] &\leq \Pr[\sum_{i=1}^T Y_i < T \rho/2]\\
        &\leq e^{-T\rho/8}\\
        &\leq \frac{1}{n}
    \end{align*}

    The first inequality holds if we take $T\geq 4en^2K_{\beta}$. The second inequality is by applying Chernoff bound and the last one holds if we take $T\geq 16enK_{\beta}\log{n}$.
    
\end{proof}
Therefore, if the algorithm takes $T\geq \max\{4en^2K_{\beta}, 16enK_{\beta}\log n\}$ iterations, it will give a  $\frac{1}{2}$ approximation solution with high probability $1-1/n$.
\end{proof}


% \begin{theorem}
%     % \label{th:dynamic-po-smaller-cost}
%     If Algorithm \ref{alg:po} has achieved a $1/2$-approximation with a cost constraint $\beta$, then for a smaller cost $b \in (0, \beta)$, the algorithm already has achieved $1/2$-approximation.
% \end{theorem}



% \begin{theorem}
%     % \label{th:dynamic-po-larger-cost}
%     If Algorithm \ref{alg:po} has achieved a $1/2$-approximation with a cost constraint $\beta$, then for a larger cost $B > \beta$, the algorithm can regain $1/2$-approximation after making $4en^2 (K_B - K_{\beta})$ more iterations.
% \end{theorem}
